Fairness in Submodular Maximization over a Matroid Constraint

Submodular maximization over a matroid constraint is a fundamental problem with various applications in machine learning. Some of these applications involve decision-making over datapoints with sensitive attributes such as gender or race. In such settings, it is crucial to guarantee that the selected solution is fairly distributed with respect to this attribute. Recently, fairness has been investigated in submodular maximization under a cardinality constraint in both the streaming and offline settings, however the more general problem with matroid constraint has only been considered in the streaming setting and only for monotone objectives. This work fills this gap. We propose various algorithms and impossibility results offering different trade-offs between quality, fairness, and generality.

==> settings/packages.tex <==
% Recommended, but optional, packages for figures and better typesetting:
\usepackage{microtype}
\usepackage{graphicx}
%\usepackage{subfigure}
\usepackage{wrapfig}
\usepackage{subcaption}
\usepackage{booktabs} % for professional tables
\setlength \cmidrulewidth{0.1pt}
%\usepackage{multirow}

\RequirePackage{algorithm}
\RequirePackage[noend]{algorithmic}
% hyperref makes hyperlinks in the resulting PDF.
\usepackage[hidelinks, pagebackref=true]{hyperref}
\renewcommand*\backref[1]{\ifx#1\relax \else (Cited on #1) \fi}

% Attempt to make hyperref and algorithmic work together better:
\newcommand{\theHalgorithm}{\arabic{algorithm}}


% For theorems and such
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsthm}
\usepackage{mathtools}
\usepackage{thm-restate}

% Other packages
\usepackage{adjustbox}
\usepackage{xspace}
\usepackage{dsfont}

% To restate Theorems
%\usepackage{apxproof} % didn't work with overleaf 
\usepackage{thmtools} 
\usepackage{thm-restate}

% if you use cleveref..
\usepackage[capitalize,noabbrev]{cleveref}

\usepackage[disable]{todonotes}
%\usepackage{todonotes}

\usepackage{enumitem}

% to cross reference footnotes
\makeatletter
\newcommand\footnoteref[1]{\protected@xdef\@thefnmark{\ref{#1}}\@footnotemark}
\makeatother
